Impact of Physical Activity on Sleep:A Deep Learning Based Exploration

The importance of sleep is paramount for maintaining physical, emotional and mental wellbeing. Though the relationship between sleep and physical activity is known to be important, it is not yet fully understood. The explosion in popularity of actigraphy and wearable devices, provides a unique opportunity to understand this relationship. Leveraging this information source requires new tools to be developed to facilitate data-driven research for sleep and activity patient-recommendations. In this paper we explore the use of deep learning to build sleep quality prediction models based on actigraphy data. We first use deep learning as a pure model building device by performing human activity recognition (HAR) on raw sensor data, and using deep learning to build sleep prediction models. We compare the deep learning models with those build using classical approaches, i.e. logistic regression, support vector machines, random forest and adaboost. Secondly, we employ the advantage of deep learning with its ability to handle high dimensional datasets. We explore several deep learning models on the raw wearable sensor output without performing HAR or any other feature extraction. Our results show that using a convolutional neural network on the raw wearables output improves the predictive value of sleep quality from physical activity, by an additional 8% compared to state-of-the-art non-deep learning approaches, which itself shows a 15% improvement over current practice. Moreover, utilizing deep learning on raw data eliminates the need for data pre-processing and simplifies the overall workflow to analyze actigraphy data for sleep and physical activity research.

==> cnn_fig.tex <==
\begin{figure}[t!]
\begin{adjustbox}{width=3.5in,totalheight=2.0in}
\begin{tikzpicture}[
%scale=0.8,
%transform canvas={scale=0.8},
plain/.style={draw=none, fill=none},
net/.style={matrix of nodes, nodes={draw, circle, inner sep=2pt, minimum size=0.2cm, anchor=center},
nodes in empty cells, column sep=0.02cm, row sep=1cm},
row 1/.style={nodes={minimum size=1cm}},
row 4/.style={nodes={minimum size=1cm}},
>=latex
]

%=======================
%==> draw NN diagram <==
%=======================

\matrix[net] (mat)
{
|[plain]| & |[plain]| & |[plain]| & y & |[plain]| \\
%|[plain]| & |[plain]| & |[plain]| & & & |[plain]| \dots & \\
|[plain]| & & & & & |[plain]| \dots & & \\
& & & & & & |[plain]| \dots & & & |[plain]| &\\ 
|[plain]| &  x$_{t-1}$ & |[plain]| &  |[plain]| &  x$_{t}$ & |[plain]| & |[plain]| \dots & |[plain]| & x$_{T}$\\ 
};
\tikzstyle{annot} = [text width=5em, text centered]

%=====================
%==> combine nodes <==
%=====================
% in the first hidden layer
\node[draw,dashed,fit=(mat-3-1) (mat-3-2) (mat-3-3)] (a1) {};
\node[draw,dashed,fit=(mat-3-4) (mat-3-5) (mat-3-6)] (a2) {};
\node[draw,dashed,fit=(mat-3-8) (mat-3-9) (mat-3-11)] (a3) {};

% in the second hidden layer
\node[draw,dashed,fit=(mat-2-2) (mat-2-3)] (b1) {};
\node[draw,dashed,fit=(mat-2-4) (mat-2-5)] (b2) {};
\node[draw,dashed,fit=(mat-2-7) (mat-2-8)] (b3) {};

% in the third hidden layer
%\node[draw,dashed,fit=(mat-2-4) (mat-2-5) (mat-2-7)] (c1) {};

%==========================
%==> define input words <==
%==========================
%\node[annot,below of=mat-5-2, node distance=1cm] (a) {medical};
%\node[annot,below of=mat-5-4, node distance=1.08cm] (b) {emergency};
%\node[annot,below of=mat-5-6, node distance=1cm] (c) {\dots};
%\node[annot,below of=mat-5-8, node distance=1cm] (d) {HTTP};

%===================================
%==> add labels to hidden layers <==
%===================================
% 1st hidden layer
\path (mat-3-1) |- (mat-3-1) node [near end,above] {h$_{i-1}$};
\path (mat-3-4) |- (mat-3-4) node [near end,above] {h$_{i}$};
\path (mat-3-10) |- (mat-3-10) node [near end,above] {h$_{N}$};

% 2nd hidden layer
\path (mat-3-2) |- (mat-2-2) node [near end,above] {m$_{i-1}$};
\path (mat-3-4) |- (mat-2-4) node [near end,above] {m$_{i}$};
\path (mat-3-8) |- (mat-2-8) node [near end,above] {m$_{N}$};

% 2nd hidden layer
%\path (mat-2-4) |- (mat-2-4) node [near end,above] {z};

%==============
%==> arrows <==
%==============
% word to input arrows
%\draw[->] (a) -- (mat-5-2);
%\draw[->] (b) -- (mat-5-4);
%\draw[->] (d) -- (mat-5-8);

\foreach \mi in {2,3} 
	{
	% from 1st hidden to 2nd hidden layer
	\draw[->] (a\mi) -- (b\mi);
	% from 2nd hidden to 3rd hidden layer
	\draw[->] (b\mi) -- (mat-1-4);
    }

% weights label
\draw[->] (a1) -- (b1);
\draw[->] (b1) -- (mat-1-4) node[left, midway] {\bf{w}};

% from 3rd hidden to output layer
%\draw[->] (c1) -- (mat-1-5) node[left, midway] {\bf{w}};

% Annotate the layers
\node[annot,left of=mat-1-1,distance=1cm,align=left] {Output layer};
%\node[annot,left of=mat-2-1,distance=1cm,align=left] {Dense layer};
\node[annot,left of=mat-2-1,distance=1cm,align=left] {Max \enspace pooling};
\node[annot,left of=mat-3-1,distance=1cm,align=left] {Feature maps};
\node[annot,left of=mat-4-1,distance=1cm,align=left] {Input vectors};

%child inheriting arrows
\foreach \mi in {1,2,3}
	{
    \node[below of=a\mi,yshift=.75cm] {}
		child[sibling distance=15mm, level distance=5mm]{}
		child[sibling distance=15mm,level distance=5mm]{}
		child[sibling distance=15mm,level distance=5mm]{};
    }
\end{tikzpicture}
\end{adjustbox}
\label{fig:cnn}
\caption{Convolutional Neural Network}
\end{figure}

==> deep_learning_models.tex <==

Let $\mathbf{x_t}\in\real^{D}$ be a vector representing a person's activity measured at time $t$. 
Given a series of such input feature vectors $\mathbf{X} = (\mathbf{x}_1, \cdots, \mathbf{x}_T)$ representing a person's physical activity in an awake time period, the deep neural models first compute compressed representations with multiple levels of abstraction by passing the inputs through one or more non-linear hidden layers. The abstract representations of the raw activity measures are then used in the output layer of the neural network to predict the sleep quality. Formally, the output layer defines a Bernoulli distribution over the sleep quality $y \in $ \{\textit{good, poor}\}:  

\begin{equation}
p(y|\mathbf{X}, \theta)= \Ber(y| \sig(\mathbf{w^T} \phi(\mathbf{X}) + b )) \label{loss}
\end{equation}

\noindent  where $\sig$ refers to the sigmoid function, $\phi(\mathbf{X})$ defines the transformations of the input $\mathbf{X}$ through non-linear hidden layers, $\mathbf{w}$ are the output layer weights and $b$ is a bias term.


We fit (or train) the models by minimizing the cross-entropy between the predicted distributions $\hat{y}_{n\theta} = p(y_n|\mathbf{X}_n, \theta)$ and the target distributions $y_n$ (i.e., the gold labels).\footnote{Other loss functions (e.g., hinge) yielded similar results.}

\begin{equation}
J(\theta) =  - \sum_{n} y_n \log \hat{y}_{n\theta} + (1-y_n) \log \left(1- \hat{y}_{n\theta} \right) \label{eq:ce}
\end{equation}

Minimizing cross-entropy is same as minimizing the negative log-likelihood (NLL) of the data (or maximizing log-likelihood). Unlike generalized linear models (e.g., logistic regression), the NLL of a deep neural model is a non-convex function of its parameters. Nevertheless, we can find a locally optimal maximum likelihood (ML) or maximum a posterior (MAP) estimate using gradient-based optimization methods. The main difference between the models, as we describe below, is how they compute the abstract representation $\phi(\mathbf{X})$.     

\subsubsection{Feed-forward Neural Network} \label{mlp}

Feed-forward Neural Networks, aka Multi-Layer Perceptrons (MLP) are the simplest models in the deep learning family. As shown in fig. \ref{fig:mlp}, the transformation of input $\phi(\mathbf{X})$ in MLP is defined by one or more fully-connected hidden layers of the form  

\begin{equation}
\phi(\mathbf{X}) =  f(V\mathbf{x_{1:T}}) = [f(\mathbf{v}_1^T\mathbf{x_{1:T}}), \cdots , f(\mathbf{v}_N^T\mathbf{x_{1:T}})]
\end{equation}

\noindent where $\mathbf{x_{1:T}}$ is the concatenation of the feature vectors $\mathbf{x}_1, \cdots, \mathbf{x}_T$, $V$ is the weight matrix from the inputs to the hidden units, $f$ is a non-linear activation function (e.g., $\sig, \tanh$) applied element-wise, and $N$ is the number of hidden units. MLP without any hidden layer (i.e., non-linear activations) boils down to a logistic regression (LR) or maximum entropy (MaxEnt) model. The hidden layers give MLP representational power to model complex dependencies between the input and the output.\footnote{In fact, MLP has been shown to be a \emph{universal approximator}, meaning that it can model any suitably smooth function to any desired level of accuracy, given the required hidden units  \cite{Hornik:1991}.} By transforming  a large and diverse set of raw activity measures into a more compressed abstract representation through its hidden layer, MLP can improve the prediction accuracy over linear models like LR. 

\begin{figure}[tb!]
\centering
%\includegraphics[height=3.65in,width=.52\textwidth]{MLP_final}
\includegraphics[scale=1.0]{MLP}
\label{fig:mlp}
\caption{A multi-layer perceptron with one hidden layer.}
\end{figure}


%\red{Image of   MLP, 
%Why it works well. 
%Why will it work well this context. 
%What are its constraints?
%Why do we expect its better than logistic regression? (cite proof if need be)
%}

\subsubsection{Convolutional Neural Network} \label{cnn}

The fully-connected MLP described above has two main properties: \Ni it composes each higher level feature from the entire input, and \Nii it is \emph{time variant}, meaning it uses separate (non-shared) weight  parameter for each input dimension to predict the overall sleep quality. However, a person's sleep quality may be determined by his activity over certain (local) time periods in the awake time as opposed to the entire awake time, and this can be invariant to specific timings. For example, high intensity exercises or games over certain period of time can lead to good sleep, no matter when the activities are exactly performed in the awake time. Furthermore, each person has his own habit of activities, e.g., some run in the morning while others run in the afternoon. A fully-connected structure would require a lot of data to effectively learn these specific activity patterns, which is rarely the case in health domain. Convolutional neural networks (CNN) address these issues of a fully-connected MLP by having repetitive filters or kernels that are applied to local time slots to compose higher level abstract features. The weights for these filters are shared across time slots. 

As shown in Fig. \ref{fig:cnn}, the hidden layers in a CNN are formed by a sequence of \textit{convolution} and \textit{pooling} operations. A convolution operation involves applying a \emph{filter} $\mathbf{u} \in \real^{L.D}$ to a window of $L$ feature vectors to produce a new feature $h_t$   
     


\begin{equation}
h_t = f(\mathbf{u} . \mathbf{x}_{t:t+L-1})
\end{equation}

\noindent where $\mathbf{x}_{t:t+L-1}$ denotes the concatenation of $L$ input vectors and  $f$ is a non-linear activation function as defined before. We apply this filter to each possible $L$-word window in the sequence $\mathbf{X}$ to generate a \emph{feature map} $\mathbf{h}^i = [h_1, \cdots, h_{T+L-1}]$. We repeat this process $N$ times with $N$ different filters to get $N$ different feature maps $[\mathbf{h}^1, \cdots, \mathbf{h}^N]$. Note that we use a \emph{wide} convolution rather than a \emph{narrow} one, which ensures that the filters reach the entire sentence, including the boundary words \cite{Kalchbrenner14}. This is done by performing \emph{zero-padding}, where out-of-range ($t$$<$$1$ or $t$$>$$T$) vectors are assumed to be zero. 

%\begin{figure}[tb!]
%\centering
%\includegraphics[height=2.2in,width=.48\textwidth]{CNN-health}
%\label{fig:cnn}
%\caption{Convolutional neural network.}
%\end{figure}

\begin{figure}[tb!]
\centering
%\includegraphics[height=3.65in,width=.52\textwidth]{MLP_final}
\includegraphics[scale=0.8]{CNN}
\label{fig:cnn}
\caption{A convolutional neural network. Each colored box in the second hidden layer represents a feature map, which is obtained by sliding its corresponding filter over the entire input. Pooling is independently done over feature maps.}
\end{figure}


%\input{cnn_fig.tex}


After the convolution, we apply a max-pooling operation\footnote{Other pooling operations are possible. In our experiments, we found max-pooling giving better results than mean-pooling.} to each feature map
%take the maximum value of  as the feature corresponding to the filter:  

\begin{equation}
\mathbf{m} = [\mu_p(\mathbf{h}^1), \cdots, \mu_p(\mathbf{h}^N)] \label{max_pool}
\end{equation}

\noindent where $\mu_p(\mathbf{h}^i)$ refers to the $\max$ operation applied to each window of $p$ features in the feature map $\mathbf{h}^i$. For $p=2$, this pooling gives the same number of features as in the feature map (because of the zero padding). 

Intuitively, the filters compose activity measures in local time slots into higher-level representations in the feature maps, and max-pooling reduces the output dimensionality while keeping the most important aspects from each feature map. Since each convolution-pooling operation is performed independently, the features extracted become invariant in locations, i.e., where they occur in the awake time. This design of CNNs yields fewer parameters than its fully-connected counterpart, therefore, generalizes well for target prediction tasks.  

%CNN captures the most salient $n$-gram information by means of its convolution and max-pooling operations.

%\red{Advantages of CNN}
%\red{Intuition: Why would we expect a CNN to work well in this context.}
%\red{What are its constraints?} 

\subsubsection{Recurrent Neural Network} \label{rnn}

In CNN, features are considered in a bag-of-words fashion disregarding the order information. The order in which the activities were performed in an awake time could be important. Recurrent neural networks (RNN) compose abstract features by processing activity measures in an awake time sequentially, at each time step combining the current input with the previous hidden state. More specifically, as depicted in Fig. \ref{fig:rnn}, RNN computes the output of the hidden layer $\mathbf{h}_t$ at time $t$ from a nonlinear transformation of the current input $\mathbf{x}_t$ and the output of the previous hidden layer $\mathbf{h}_{t-1}$. More formally,

\begin{equation}
\mathbf{h}_t = f( U \mathbf{h}_{t-1} + V \mathbf{x}_t) \label{rec}
\end{equation}

\noindent where $f$ is a nonlinear activation function as before, and $U$ and $V$ are compositional weight matrices. RNNs create internal states by remembering previous hidden layer, which allows them to exhibit dynamic temporal behavior. We can interpret $\mathbf{h}_t$ as an intermediate representation summarizing the past. The representation for the entire sequence can be obtained by performing a pooling operation (e.g., \emph{mean-pooling, max-pooling}) over the sequence of hidden layers or simply by picking the last hidden layer $\mathbf{h}_T$. In our experiments, we found mean-pooling to be more effective than other methods.     

%\begin{figure}[tb!]
%\centering
%\includegraphics[height=3.65in,width=.52\textwidth]{MLP_final}
%\includegraphics[scale=0.9]{RNN}
%\label{fig:rnn}
%\caption{A recurrent neural network.}
%\end{figure}


\begin{figure*}[t!]
\centering
%\subfigure[Convolution neural network.]{%
%\includegraphics[height=1.8in,width=.38\textwidth]{cnn-newest-5.png}
%\label{fig:cnn}}
%\quad
\subfigure[]{%
\includegraphics[scale=0.84]{RNN}
\label{fig:rnn}}
\quad
\subfigure[]{
%\raisebox{20mm}{\includegraphics[height=1.35in,width=.28\textwidth]{lstm.png}}
\raisebox{20mm}{\includegraphics[scale=0.4]{lstm.png}}
\label{fig:lstm}}
\caption{ (a) A recurrent neural network with one recurrent layer, and (b) an LSTM memory block, which represents a hidden unit in an LSTM-RNN.}
\end{figure*}


%The last hidden layer  thus represents the whole input sequence, which is fed to the output layer for classification (i.e., $\mathbf{z} = \mathbf{h}_T$). 


%For example, \red{give an intuitive example}

RNNs are generally trained with the backpropagation through time (BPTT) algorithm, where errors (i.e., gradients) are propagated back through the edges over time. One common issue with BPTT is that as the errors get propagated, they may soon become very small or very large that can lead to undesired values in weight matrices, causing the training to fail. This is known as the \emph{vanishing} and the \emph{exploding} gradients problem \cite{Bengio:1994}. One simple way to overcome this issue is to use a truncated BPTT \cite{Mikolov12} for restricting the backpropagation to only few steps like $4$ or $5$. However, this solution limits the simple RNN to capture long-range dependencies. Below we describe an elegant RNN architecture to address this problem.       


\paragraph*{Long Short-Term Memory RNN}
Long short-term memory or LSTM \cite{Hochreiter:1997} is specifically designed to capture long range dependencies in RNNs. The recurrent layer in a standard LSTM is constituted with special units called \emph{memory blocks} (Fig. \ref{fig:rnn} and \ref{fig:lstm}). A memory block is composed of four elements: \Ni a memory cell $c$ (a neuron) with a self-connection, \Nii an input gate $i$ to control the flow of input signal into the neuron, \Niii an output gate $o$ to control the effect of the neuron activation on other neurons, and \Niv a forget gate $f$ to allow the neuron to adaptively reset its current state through the self-connection. The following sequence of equations describe how the memory blocks are updated at every time step $t$: 

%More  formally, %LSTM RNN performs 
\begin{eqnarray}
	\mathbf{i}_t &=& \sigh(U_i\mathbf{h}_{t-1} + V_i\mathbf{x}_t + \mathbf{b}_i)  \label {lstm_first}\\
    \mathbf{f}_t &=& \sigh(U_f\mathbf{h}_{t-1} + V_f\mathbf{x}_t + \mathbf{b}_f) \\
    \mathbf{c}_t &=& \hspace{-0.1cm}  \mathbf{i}_t\odot \tanh(U_c\mathbf{h}_{t-1} + V_c\mathbf{x}_t) + \mathbf{f}_t\odot\mathbf{c}_{t-1} \\
    \mathbf{o}_t &=& \sigh(U_o\mathbf{h}_{t-1} + V_o\mathbf{x}_t + \mathbf{b}_o) \\
    \mathbf{h}_t &=& \mathbf{o}_t \odot \tanh(\mathbf{c}_t) \label {lstm_last}
%    y_t &=& W_{hy}h_t + b_y
\end{eqnarray}

\noindent where $U_k$ and $V_k$ are the weight matrices between two consecutive hidden layers, and between the input and the hidden layers, respectively, which are associated with gate $k$ (input, output, forget and cell); and and $\mathbf{b}_k$ is the corresponding bias vector. The symbols $\sigh$ and $\tanh$ denote hard sigmoid and hard tan, respectively, and the symbol $\odot$ denotes a element-wise product of two vectors. LSTM by means of its specifically designed gates (as opposed to simple RNNs) is capable of capturing long range dependencies.



\paragraph*{Sequence Construction in RNNs}

The obvious way to apply RNNs to activity records is to consider the accelerometer output at every \red{minute?} in an awake time as a separate time step. In our data, each time step contains only one measure (i.e., the vertical axis) and the maximum length of a sequence is $2470$ with an average of \red{$xxx$}. This results in very lengthy sequences with only one feature at each time step. RNNs applied to this setting suffer from two problems: \Ni because of the low dimensional input (e.g., 1 in our case) at each time step, RNNs become ineffective in composing features and fail to capture the sequential dependencies, and \Nii because of long sequences, the gradients (errors) from the final time step vanish before they reach to earlier parts of the network, causing the training with BPTT to fail even with LSTM cells. 

To circumvent this problem, we construct pseudo time steps by merging accelerometer measures over $S$ time steps. In other words, each pseudo time step in this setting generates an input vector of $S$ elements. To make all input vectors equal-sized, we use zero-padding for the last time step (if needed). Note that setting $S=1$ gives the original sequences. In our experiments, we experimented with $S \in \{25, 50, 75, 100\}$.



